Bayesian Formal Synthesis of Unknown Systems via Robust Simulation Relations

This paper addresses the problem of data-driven computation of controllers that are correct by design for safety-critical systems and can provably satisfy (complex) functional requirements. With a focus on continuous-space stochastic systems with parametric uncertainty, we propose a two-stage approach that decomposes the problem into a learning stage and a robust formal controller synthesis stage. The first stage utilizes available Bayesian regression results to compute robust credible sets for the true parameters of the system. For the second stage, we introduce methods for systems subject to both stochastic and parametric uncertainties. We provide simulation relations for enabling correct-by-design control refinement that are founded on coupling uncertainties of stochastic systems via sub-probability measures. The presented relations are essential for constructing abstract models that are related to not only one model but to a set of parameterized models. The results are demonstrated on three case studies, including a nonlinear and a high-dimensional system.

==> DDSimRelSysId.tex <==
% !TEX root =  main.tex
%\color{blue!70!black}
\subsection{Data-driven simulation relations for linear systems}
Consider the following uncertain linear system
\begin{equation}\label{eq:sysDataGenLin}
	\M(\theta): \left\{\begin{array}{ll}
		x_{k+1} &= A(\theta)x_{k}+ B(\theta)u_k+ B_ww_k\\
		y_k &= Cx_k,%+D_vv_k,
	\end{array}\right.
\end{equation}
with parametrized matrices $A(\theta)\in\R^{n\times n}$, $B(\theta)\in\R^{n\times m}$, known matrices $B_w\in\R^{n\times q}$, $C$, uncertain parametrization $\theta\in\Theta$,
and the nominal model
\begin{equation}\label{eq:sysInfLin}
	\Mh: \left\{\begin{array}{ll}
		\hat x_{k+1} &= \hat{A}\hat x_{k}+ \hat{B}\hat u_k+ B_w\hat w_k\\
		\hat y_k &= C\hat x_k,
	\end{array}\right.
\end{equation}
where we abbreviate $\Mh:=\M(\hat{\theta})$, $\hat{A}:=A(\hat{\theta})$, and $\hat{B}:=B(\hat{\theta})$ for some estimate $\hat\theta$.
\red{Let the system $\M(\theta)$ be fully controllable.} \pdfmargincomment{Birgit: Why controllable? Doesn't it make more sense to require observability here instead?
Oliver: From what I got, this is required by system identification.}
Without loss of generality,
%\pdfmargincomment{If the covariance matrix is not full rank, this should only impact the coupling part where you have to take the pseudo inverse.}
we assume that the process
%and measurement noises 
noises
$w_k,\hat w_k\sim\mathcal{N}(0,\sigma_w^2I)$
%and $v_k\sim\mathcal{N}(0,\sigma_v^2I)$\pdfmargincomment{Is it fine to use $v_k$ here despite $v$ being used for the sub-probability coupling?!} 
have Gaussian distribution with a full rank covariance matrix, with variance $\sigma_w^2$ and $I$ being the identity matrix.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\medskip
\subsubsection{Robust parameter estimation}\label{sec:simRelLinEst}
Let data $\mathcal{D}$ as in \eqref{eq:data} \Birgit{be obtained from experiments}.
Here, we use the data-driven parameter identification method from \cite{Zheng2020IdentLinSys} to obtain $\hat\theta$ and $\Theta$ from $\mathcal{D}$. In the following, we reproduce the relevant results from \cite{Zheng2020IdentLinSys} and \Birgit{formulate Thm.~\ref{thm:paraId}} to derive a valid control refinement for systems \eqref{eq:sysDataGenLin}-\eqref{eq:sysInfLin} based on data $\mathcal{D}$.

We construct a function $G(\theta)$ using the first $T$ Markov parameters of the system:
\begin{align}\label{eq:Gmatrix}
	G(\theta) &= C\begin{bmatrix} B(\theta) & AB(\theta) & \ldots & [A(\theta)]^{T-2}B(\theta) \end{bmatrix},% \in \R^{p\times m(T-1)},
\end{align}
%\pdfmargincomment{Remove the dimensionsin R?}
and a function of the noise dynamics
\begin{equation*}
	F(\theta) = C\begin{bmatrix} B_w & A(\theta)B_w & \ldots & [A(\theta)]^{T-2}B_w \end{bmatrix},% \in \R^{p\times q(T-1)},
\end{equation*}
that can be upper bounded, i.e., $||F(\theta)||\leq \tilde{d}$, with some known $\tilde{d}$.
Furthermore, we define the upper-triangular Toeplitz matrix of $u^{(i)}$ as
\begin{equation*}
	U^{(i)} = \begin{bmatrix} 
		u^{(i)}_0 & u^{(i)}_1& \ldots & u^{(i)}_{T-2}\\
		0 & u^{(i)}_0 & \ldots & u^{(i)}_{T-3}\\
		\vdots & \vdots & \ddots & \vdots\\
		0 & 0 & \ldots & u^{(i)}_{0}
	\end{bmatrix},% \in \R^{m(T-1)\times (T-1)},
\end{equation*}
and summarize the data into matrices $Y, U$ as follows:
\begin{align}
	Y &= \begin{bmatrix} \bar y^{(1)} & \ldots & \bar y^{(N)} \end{bmatrix},% \in \R^{p\times N(T-1)}
	\label{eq:Ymatrix}\\
	U &= \begin{bmatrix} U^{(1)} & \ldots & U^{(N)} \end{bmatrix}% \in \R^{m(T-1)\times N(T-1)}
	\label{eq:Umatrix},
\end{align}
where $\bar y^{(i)} = y^{(i)}_1,\ldots,y^{(i)}_{T-1}$.
Using the previously defined matrices and matrix equations we give the following definition:
%stipulate the \emph{least square estimate} $\hat{G}$ minimizing the estimation error $||G(\theta^\ast)-\hat{G}||$.
%The following definition is based on \cite{Zheng2020IdentLinSys}.
\begin{definition}[Least square estimator (LSE)]\label{def:LSE}
	For the systems \eqref{eq:sysDataGenLin}-\eqref{eq:sysInfLin} with $G$ in \eqref{eq:Gmatrix}, the \emph{least square estimator} minimizing the estimation error $||G(\theta^\ast)-\hat{G}||$ is given by
	\begin{equation}\label{eq:LSE}
		\hat{G}=YU^\dagger, 
	\end{equation}
	where $Y, U$ as in \eqref{eq:Ymatrix}-\eqref{eq:Umatrix} and the right pseudo inverse of $U$ given by $U^\dagger:=U\T\left(UU\T\right)^{-1}$.
\end{definition}
Note that we infer $\hat\theta$ as the solution to $G(\hat\theta)\equiv\hat G$ with $G(\hat\theta)$ in Eq.~\eqref{eq:Gmatrix}.
Based on \cite{Zheng2020IdentLinSys}, Theorem~3.1 we obtain a confidence set $\Theta$ using the confidence bound given in the following proposition. 
%For this, the authors \textsl{Zheng et al.} implicitly raise the following assumption:
%\begin{assumption}\label{asm:boundsOnF}
%	There exists a known bound $||F(\theta^\ast)||$.
%\end{assumption}
Like the authors \textsl{Zheng et al.} we set $||F(\theta^\ast)||\approx||F(\hat\theta)||$.
\begin{proposition}[Confidence bound]\label{prop:confbound}
	Let $N$ data sequences with $N\geq8mT+4(m+q+4)\log(\frac{3T}{\alpha})$\pdfmargincomment{Must include all the explanations for the parameters when defining the model.} for some $\alpha\in(0,1)$ \Birgit{be given}. \pdfmargincomment{Birgit: Unclear. What are $m$ and $q$? Oliver: Defined when introducing the models in the beginning of this subsection. Is this too subtle?} Then, we can upper bound the estimation error as
	\begin{equation}
		\P\left(||{G}(\hat\theta)-G(\theta^\ast)||\leq\frac{\sigma_wC}{\sigma_u\sqrt{N}}\right)\geq 1-\alpha,\label{eq:confidence_bound}
	\end{equation}
%	\begin{equation}
%		\P\left(||{G}(\hat\theta)-G(\theta^\ast)||\leq\frac{\sigma_vC_1+\sigma_wC_2}{\sigma_u\sqrt{N}}\right)\geq 1-\alpha,\label{eq:confidence_bound}
%	\end{equation}
	with constant
	\begin{equation}
		C := 16||F||\sqrt{\left(\frac{T^3}{3}+\frac{T^2}{2}+\frac{T}{6}\right)(m+q)\log\left(\frac{27T}{\alpha}\right)}.\label{eq:C2}
	\end{equation}
%	\begin{align}
%		C_1 &:= 8||D_v||\sqrt{2T(T+1)(m+l)\log\left(\frac{27T}{\alpha}\right)}\text{ and}\label{eq:C1}
%		\\
%		C_2 &:= 16||F||\sqrt{\left(\frac{T^3}{3}+\frac{T^2}{2}+\frac{T}{6}\right)(m+q)\log\left(\frac{27T}{\alpha}\right)}.\label{eq:C2}
%	\end{align}
\end{proposition}
Note that the estimation error $||{G}(\hat\theta)-G(\theta^\ast)||$  behaves as $\mathscr{O}(\sqrt{N}^{-1})$. \pdfmargincomment{Birgit: I am not familiar with the big-O-notation, so I am not sure if this can be expected from the reader.} We obtain the confidence set $\Theta$ by fixing $\hat\theta$ to be the LSE from Def.~\ref{def:LSE} and solving \eqref{eq:confidence_bound} for $\theta^\ast$.


%\red{Is this correct?!:} We recover the confidence bounds $||\hat{A}-A||\leq||\hat{G}-G||$ and $||\hat{B}-B||\leq||\hat{G}-G||$.

\begin{algorithm}
	\caption{Robust parameter estimation \cite{Zheng2020IdentLinSys}}
	\begin{algorithmic}[1]  % Add [1] for line numbers 
		\REQUIRE Data $U,Y$, desired confidence level $1-\alpha$
		\ENSURE Estimate $\hat \theta$, robust confidence set $\Theta$
		\STATE Calculate LSE $\hat G\gets YU^\dagger$
		\STATE Obtain nominal $\hat\theta$ solving $G(\hat\theta)\equiv\hat G$
		\STATE Compute constant $C\gets\eqref{eq:C2}$
		\STATE Obtain $\Theta$ as solution to \eqref{eq:confidence_bound} by solving for $\theta^\ast$
	\end{algorithmic}
\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Valid control refinement}
Now, we want to find a valid control refinement based on the estimated parameters.
\color{black} 
%\pdfmargincomment{Birgit: Introduce this part. At the moment it comes as a surprise. Oliver: Done.}
The probability of transitioning from a state $x_k$ with input $u_k$ to a state $x_{k+1}\in S$ is given by $P(x_{k+1}\in S|x_k,u_k) = \int_{S} \Tr(dx_{k+1}|x_k,u_k)$, where
\begin{align}
	\begin{split}
		\Tr(\dxp|x,u;\theta) &= \mathcal N(\dxp|A(\theta)x+B(\theta)u, I)\\
		&	= \int_w \fdel{\dxp|w;\theta} \mathcal N(dw|0, I).
	\end{split}\label{eq:tr}
\end{align}
In this equation,  $\mathcal N$ and $f_\delta$ are the normal and Dirac stochastic kernels defined by
\begin{align}
	&\mathcal N(\dxp|m, \Sigma) \!:=\!\frac{\dxp}{ \sqrt{(2\pi)^n \!\left|\Sigma\right| }}\exp\!\left[\!-\frac{1}{2}(x^+\!\!\!-\!m)\T\!\Sigma^{-1}\!(x^+\!\!\!-\!m)\!\right]\nonumber\\
	& \fdel{\dxp|w;\theta}:= \delta_{A(\theta)x+B(\theta)u+B_ww}(\dxp),
	\label{eq:fdel_lin}
\end{align}
with $n := \mathrm{dim}\left(\Sigma\right)$ and $|\Sigma|$ the determinant of $\Sigma$. \pdfmargincomment{Birgit: Also explain what Sigma $\Sigma$ itself represents. This has not been introduced in the paper yet. Same holds for $m$. Also make sure that it is not an issue that in  the beginning of this section (IVA) you denote  the variance as $\sigma^2_wI$.}

Similarly, the stochastic kernel of $\Mh$ is
\begin{align}
	\begin{split}
		\hat\Tr(\dxhp|\hat x,\hat u)& = \mathcal N(\dxhp|\hat A\hat x+\hat B\hat u, I)\\
		&	= \int_{\hat w} \fhdel{\dxhp|\hat w} \mathcal N(d\hat w|0, I),\text{ with}
	\end{split}\label{eq:tr_hat}\\
	\fhdel{\dxhp|\hat w}&:=\delta_{\hat A\hat x+\hat B\hat u+B_w\hat w}(\dxhp).
	\label{eq:fhdel_lin}
\end{align}

Note that $\fdel{\cdotx}$ and $\fhdel{\cdotx}$ are dependent on $x,u$, and $\hat x,\hat u$, respectively, omitted here for conciseness.

\color{blue!70!black}
We can rewrite the model in Eq.~\eqref{eq:sysDataGenLin} as
\begin{equation*}
	x_{k+1} =\underbrace{\hat Ax_{k}+\hat Bu_k}_{\text{nominal dynamics}} + \underbrace{(A(\theta)-\hat A)x_{k}+ (B(\theta)-\hat B)u_k+B_ww_k}_{\text{disturbance}}.
\end{equation*}
Note that the disturbance part consists of a deviation caused by the unknown parameter $\theta$ and a deviation caused by the noise $w_k$.
Let us assume that we can bound the former as
\begin{equation}
	%\label{eq:bound_offset}
	\|(A(\theta)-\hat A)x+ (B(\theta)-\hat B)u\|\leq d(x, u)\quad  \forall x, u,  \theta.\pdfmargincomment{Comma before "for all" symbol?}
	\label{eq:disturbance_bound_lin}
\end{equation}
We choose the interface function $\ac{k}\sim\InF(\cdotx|\hat x_k, x_k, \hat u_k):=\ach{k}$ and the noise coupling %\pdfmargincomment{Birgit: I believe it is important to make a Remark about the fact that we require $B_w$ to be invertible. Perhaps even early in the paper.}
\begin{align}
	& \hat w_k \equiv \gamma(x_k, u_k,\theta;\hat\theta)+w_k \,\,\text{ with }\nonumber\\
	& \gamma(x, u,\theta;\hat\theta) :=  B_w^{-1}(A(\theta)-\hat{A})x+ B_w^{-1}(B(\theta)-\hat{B})u,\label{eq:gamma_paraId}
\end{align}
to get the state mapping
\begin{equation}
		\label{eq:statemap_paraId}
	\xhp = \xp-\hat{A}(x_k-\hat x_k)-\hat{B}(\ac{k}-\ach{k}).
\end{equation}
not dependent on $\theta$, i.e., 
\begin{equation}
	\label{eq:statemap}
	\xhp \sim \Refi(\cdotx |\xh{k}, \x{k}, \x{k+1},\ach{k}) := \delta_{\xp-\hat A x^\Delta_k-\hat B u^\Delta_k}(d\xhp),
\end{equation}
where $x^\Delta_k:=x_k-\hat x_k$ and $u^\Delta_k:=\ac{k}-\ach{k}$.
Note that if $B_w$ is not invertible, i.e., because of rank-deficient noise, we use its pseudo inverse instead.  \pdfmargincomment{Birgit: Are you 100\% sure that the method still works if Bw is not invertible? If I use Bw = [1 0; 0 0] and multiply with its pseudo-inverse in Matlab, I obtain [1 0; 0 0] as a result. So the theta-dependent terms will not dissapear right?
Oliver: Maybe I should add a remark somewhere with all the information about this together. To make it clear, all state variables with parametric uncertainty need to be impacted by noise. If there is a state variable without parametric uncertainty AND noise, this is fine and we just take the pseudo-inverse.}
To establish an SSR $\widehat{\M}\preceq^{\delta}_\eps\M(\theta)$, we select the relation
\begin{equation}
	\label{eq:relation_linear}
	\R:=\{ (\hat x,x)\in\Xh\times\X \given x=\hat x\}.
\end{equation}
Condition (a) of Def.~\ref{def:subsim} holds by setting the initial states $\hat x_{0} = x_{0}$. Condition (c) is satisfied with $\eps=0$ since both systems use the same output mapping.
%\pdfmargincomment{Is this still true with the added measurement noise?!}. 
For condition (b), we define the sub-probability coupling $\Wt(\cdotx|\theta)$ of $\hat \Tr(\cdotx|\hat x,\ach{})$ and $\Tr(\cdotx|x,\InF;\theta)$ over $\R$:
\begin{align}
	%	\begin{split}
		&\Wt(d\xhp\times d\xp|\theta) =  \int_{\hat w}\int_w \fhdel{\dxhp|\hat w} \fdel{\dxp|w;\theta}\label{eq:subprobcoup_paraID} \\
		&\hspace{30pt}\times \delta_{\offset+w}(d\hat w) \min\{\mathcal N(dw|0,I),\mathcal N(dw|-\offset, I)\},\nonumber
		%	\end{split}
\end{align}
that takes the minimum of two probability measures. Note that we dropped the arguments of $\offset$ to lighten the notation.

\begin{theorem}\label{thm:paraId}
	For the linear models in \eqref{eq:sysDataGenLin}-\eqref{eq:sysInfLin} and some $\alpha\in(0,1)$ we have that   \pdfmargincomment{Birgit: The points a and b are hard to read. Are there some words missing?}
	\begin{itemize}
		\item[a)]  $\hat\theta$ \Birgit{is} the LSE minimizing $||G(\hat\theta)-G(\theta^\ast)||$ (Def.~\ref{def:LSE});
		\item[b)]  $\Psi$ s.t. $\P(||{G}(\hat\theta)-G(\theta^\ast)||\leq \Phi
		)\geq 1-\alpha$ (Prop.~\ref{prop:confbound}); and
		\item[c)]  $\widehat{\M}\preceq^{\delta}_\eps\M(\theta)$ with interface function $\ac{k} = \ach{k}$, relation \eqref{eq:relation_linear}, and the sub-probability kernel \eqref{eq:subprobcoup_paraID}.
	\end{itemize}
	 The state mapping \eqref{eq:statemap_paraId} defines a valid control refinement with $\eps=0$ and
	\begin{align}
		\begin{split}
			\delta(x, u; \hat\theta) = &\max_{\theta} \left\lbrace 1-2\cdot\cdf{-\frac{1}{2}\norm{\gamma(x, u,\theta;\hat\theta)}}\right\rbrace\\
			&\text{s.t.}\quad ||{G}(\hat\theta)-G(\theta)|| \leq\Phi,
		\end{split}\label{eq:delta_ddlinear}
	\end{align}\pdfmargincomment[]{Should I remove argument hattheta?}
	with a confidence of $1-\alpha$, where $\cdf{\cdot}$ is the cumulative distribution function of a Gaussian distribution, $\cdf{\zeta}:= \int_{-\infty}^\zeta \frac{1}{\sqrt{2\pi}}\exp(-\beta^2/2)d\beta$ \new{and $\offset$ as defined in \eqref{eq:gamma_paraId}}.  
%	\pdfmargincomment{Birgit: Why use alpha again in the cdf? Oliver: Done.}
\end{theorem}
\begin{proof}
	The proof of Thm.~\ref{thm:paraId} is deferred to App.~XXX. 
	This proof is similar to the proof of Thm.~\ref{thm:nonlinear} in App.~\ref{app:proofSSRnonlinear}.
	Analogously, we get $\gamma(x, u,\theta;\hat\theta)=0$ for all $\theta\in\Theta$, $(x,u)\in\X\times\U$. Using $\Theta=\{\theta\in\R^\mathfrak{p}\given||{G}(\hat\theta)-G(\theta)|| \leq\Phi\}$
	we obtain \eqref{eq:delta_ddlinear}.
\end{proof}

\color{blue!70!black}
\smallskip
\noindent\textbf{Visualization of the sub-probability coupling:}
We can reduce Eq.~\eqref{eq:subprobcoup_paraID} to
\begin{align*}
	&\Wt(d\xhp\times d\xp|\theta) = \int_{\hat w} \delta_{\xhp}(d\xp) \fhdel{\dxhp|\hat w}\\
	&\hspace{100pt}\times \min\{\mathcal N(d\hat w|\offset,I),\mathcal N(d\hat w|0, I)\}.
\end{align*}
This coupling is constructed based on the sub-probability coupling of the noises
\begin{align*}
	&\bar{{w}}( d\hat w\times d w|\theta) := \delta_{\offset+w}(d\hat w) \\
	&\hspace{90pt}\times \min\{\mathcal N(dw|0,I),\mathcal N(dw|-\offset, I)\},
\end{align*}
%\Oliver{Deal with bold notation.}
where $\offset$ quantifies the offset of the two noise distributions. 
%The noise coupling is illustrated in Fig.~\ref{fig:gaussplot} in two dimensional space.
The resulting sub-probability coupling from Eq.~\eqref{eq:subprobcoup_paraID} is illustrated in Fig.~\ref{fig:subprobcoup}.
%\input{Gaussplot}
\input{SPCplot}
\new{\begin{remark}
	With the approach presented in this paper, parametric uncertainty is compensated by diverging the noise distributions of the systems. Hence, parametric uncertainty can only be compensated on perturbed state variables.  \pdfmargincomment{Birgit: This is due to the fact that we need Bw to be invertible. So the pseudo-inverse does not work, right? This is confusing, since earlier you mention that if Bw is not invertible, then we take the pseudo-inverse.}
\end{remark}}

\color{blue!70!black}
\subsection{Data-driven simulation relations for nonlinear systems}
Here, we consider nonlinear systems that are linear in the unknown parameters $\theta=[\theta_1,\ldots,\theta_n]\T\in\Theta\subset\R^{n\times M}$, i.e.,
\begin{equation}
	\label{eq:sysDataGenNonlin}
	\M(\theta): \left\{ \begin{array}{ll}
		x_{k+1} &= \theta f(x_k, u_k)+w_k\\
		y_k &= \red{x_k},%+D_vv_k,
	\end{array} \right.
\end{equation}
where $f:\X\times\U\rightarrow\R^M$ is known,
and the nominal model
\begin{equation}
	\label{eq:sysInfNonlin}
	\Mh: \left\{ \begin{array}{ll}
		\hat x_{k+1} &= \hat\theta f(\hat x_k, \hat u_k)+\hat w_k\\
		\hat y_k &= \red{\hat x_k}.
	\end{array} \right.
\end{equation}
with parameter estimate $\hat\theta$.
Assume that $w_k,\hat w_k\sim \mathcal N(0,\sigma_w I)$ with variance $\sigma_w$. 
Note that $f:=[f_1,\ldots,f_M]\T$ can be a comprehensive library of functions.

\subsubsection{Robust parameter estimation}\label{sec:simRelNonLinEst}
If we have prior knowledge of the unknown parameters $\theta$, we can include this in their prior probability distribution $p(\theta_i)=\mathcal{N}(m_{0,i},S_{0,i})$. Otherwise, we choose a standard normal distribution.
Based on this prior distribution, \emph{Bayesian linear regression} (e.g., \cite{Bishop2006ML}, Sec.~3.3) allows us to write the posterior distribution of the unknown parameters as
\begin{equation}\label{eq:posterior}
	p(\theta_i\given Y_i) = \mathcal N(m_{N,i}, S_{N,i}),
\end{equation}
where $Y := [Y_1,\ldots,Y_n] := [y_1,\ldots,y_N]\T$ and
where the mean and covariance are given by
\begin{align}
	m_{N,i}&:=S_{N,i}(S_{0,i}^{-1}m_{0,i}+\sigma_w^{-1}\Phi\T Y_i) \text{ and}\label{eq:mean}\\
	S_{N,i}^{-1}&:=S_{0,i}^{-1}+\sigma_w^{-1}\Phi\T\Phi,\label{eq:covariance}
\end{align}respectively. The design matrix $\Phi$ is defined as
\begin{equation*}
	\Phi := \begin{bmatrix}
		f_1(x_1) & \hdots & f_M(x_1) \\
		\vdots & \ddots & \vdots \\
		f_1(x_N) & \hdots & f_M(x_N)
	\end{bmatrix}.
\end{equation*}
%Note that $\hat\theta=[m_{N,1},\ldots,m_{N,n}]\T$. 

We pick a desired lower confidence bound $1-\alpha$ and obtain the corresponding confidence set as
\begin{align}
	\begin{split}
		\Theta &= \{\theta\in\R^{n\times M} \given (\theta_i-m_{N,i})\T S_{N,i}^{-1}(\theta_i-m_{N,i})\\ &\hspace{80pt}\leq F^{-1}(1-\alpha\given n),\,i=1,\ldots,n\},
	\end{split}\label{eq:confidenceSetNL}
\end{align}
where $F^{-1}(p\given \nu):=\{x:F(x\given\nu)=p\}$ denotes the inverse cumulative density function of the chi-square distribution $F(x\given\nu):=\int_{0}^{x}\frac{t^{(\nu-2)/2}e^{-t/2}}{2^{\nu/2}\Gamma(\nu/2)}dt$
%\frac{1}{\Gamma(p/2)}\gamma(\frac{p}{2},\frac{y}{2})$ 
with $\nu$ degrees of freedom and $\Gamma(\cdotx)$ denoting the Gamma function \red{\cite{Chew1966ConfidenceMVN}}\pdfmargincomment{Do not have access to this reference and got this from https://eprints.lancs.ac.uk/id/eprint/87557/1/StatMed_2017_penultimate.pdf.}.
% Here, we denote the gamma function as $\Gamma(\cdot)$ and the lower incomplete gamma function as $\gamma(\cdot)$.

\subsubsection{Valid control refinement}
We can rewrite the model in Eq.~\eqref{eq:sysDataGenNonlin} as
\begin{equation*}
	x_{k+1} =\underbrace{\hat\theta f(x_k, u_k)}_{\text{nominal dynamics}} + \underbrace{\theta f(x_k, u_k)-\hat\theta f(x_k, u_k)+w_k}_{\text{disturbance}}.
\end{equation*}
Note that the disturbance part consists of a deviation caused by the unknown parameter $\theta$ and a deviation caused by the noise $w_k$.
Let us assume that we can bound the former as
\begin{equation*}
	%\label{eq:bound_offset}
	\|\theta f(x, u)-\hat\theta f(x, u)\|\leq d(x, u)\quad  \forall x, u,  \theta.\pdfmargincomment{Comma before "for all" symbol?}
	%	\label{eq:disturbance_bound}
\end{equation*}
\color{blue!70!black}
Using the interface function $\ac{k} = \ach{k}$ and the noise coupling
\begin{align}
	& \hat w_k \equiv  \gamma(x, u,\theta;\hat\theta)+w_k \,\,\text{ with }\nonumber\\
	& \gamma(x, u,\theta;\hat\theta) :=
	(\theta-\hat\theta)f(x_k,u_k),\label{eq:gamma_paraId_nonlin}
\end{align}
we get the state mapping
\begin{equation}
	\label{eq:statemap_paraId_nonlin}
	\xhp = \xp-\hat\theta f(x,u)+\hat\theta f(\hat x,\hat u),
\end{equation}
that is not dependent on $\theta$.
To establish an SSR $\widehat{\M}\preceq^{\delta}_\eps\M(\theta)$, we select the identity relation \eqref{eq:relation_linear}.
Condition (a) of Def.~\ref{def:subsim} holds by setting the initial states $\hat x_{0} = x_{0}$. Condition (c) is satisfied with $\eps=0$ since both systems use the same output mapping. For condition (b), we define the sub-probability coupling $\Wt(\cdotx|\theta)$ over $\R$:
\begin{align}
	%	\begin{split}
		&\Wt(d\xhp\times d\xp|\theta) =  \int_{\hat w}\int_w \fhdel{\dxhp|\hat w} \fdel{\dxp|w;\theta}\label{eq:subprobcoup_paraID_nonlin} \\
		&\hspace{30pt}\times \delta_{\offset+w}(d\hat w) \min\{\mathcal N(dw|0,I),\mathcal N(dw|-\offset, I)\},\nonumber
		%	\end{split}
\end{align}
that takes the minimum of two probability measures. Note that we dropped the arguments of $\offset$ to lighten the notation.

\begin{theorem}\label{thm:paraId_nonlin}
	For the nonlinear models in \eqref{eq:sysDataGenNonlin}-\eqref{eq:sysInfNonlin}, we have that 
	\begin{itemize}
		\item[a)]  $\hat\theta=[m_{N,1},\ldots,m_{N,n}]\T$ (Eq.~\eqref{eq:mean});
		\item[b)]  $\Theta$ as in \eqref{eq:confidenceSetNL} with \eqref{eq:mean}-\eqref{eq:covariance}; and
		\item[c)]  $\widehat{\M}\preceq^{\delta}_\eps\M(\theta)$ with interface function $\ac{k} = \ach{k}$, relation \eqref{eq:relation_linear}, and the sub-probability kernel \eqref{eq:subprobcoup_paraID_nonlin}.
	\end{itemize}
	The state mapping \eqref{eq:statemap_paraId_nonlin} defines a valid control refinement with $\eps=0$ and
	\begin{equation}
		%		\begin{split}
			\delta(x, u; \hat\theta;\theta) = \sup_{\theta\in\Theta}\left\lbrace 1-2\cdot\cdf{-\frac{1}{2}\norm{\gamma(x, u,\theta;\hat\theta)}} \right\rbrace 
			%		\end{split}
		\label{eq:delta_ddnonlinear}
	\end{equation}
	where $\offset$ defined in \eqref{eq:gamma_paraId_nonlin}
	%	and
	%	\begin{align*}
		%		\begin{split}
			%			\tilde\theta = &\arg\max_{\theta}  \norm{\theta-\hat\theta}\\
			%		&\text{s.t.}\quad \forall i=1,\ldots,n:\,\red{p(\theta_i\given Y_i)} \geq \alpha,
			%	\end{split}
		%\end{align*}\pdfmargincomment{Wrong!}
		with a confidence of $1-\alpha$.
	\end{theorem}
	\begin{proof}
		The proof of Thm.~\ref{thm:paraId_nonlin} is deferred to App.~\ref{app:proofSSRnonlinear}.
		This proof is similar to the proof of Thm.~\ref{thm:nonlinear} in App.~\ref{app:proofSSRnonlinear}.
		Analogously, we get $\gamma(x, u,\theta;\hat\theta)=0$ for all $\theta\in\Theta$, $(x,u)\in\X\times\U$. Using $\Theta=\{\theta\in\R^\mathfrak{p}\given p(\theta_i\given Y_i) \geq \alpha, \forall i=1,\ldots,n\}$ and recognizing that $\cdf{}$ is a monotone function
		we obtain \eqref{eq:delta_ddnonlinear}.
	\end{proof}
	
	This theorem gives a $\delta$ that depends on $(\xh{k},\ach{k})$. The supremum of this quantity over $\Xh\times\Uh$ could be obtained to get a constant global $\delta$, which is more conservative.

==> DDSystemId.tex <==
\subsection{Data-driven system identification}
\begin{comment}
	%In order to infer 
	%In this work, we reformulate the unknown true system $\M^\ast$ of arbitrary form into a parametrized system $\M(\theta^\ast)$ of known or chosen form, where the true parametrization $\theta^\ast$ is unknown.
	We consider discrete-time nonlinear systems perturbed by additive stochastic noise parametrized with some parameter $\theta$:\pdfmargincomment{Can't we handle multiplicative stochastic noise as well?}
	%This modeling formalism is essential if we can only access an uncertain model of this stochastic system.\pdfmargincomment{Can't we handle multiplicative stochastic noise as well?}
	%Consider the model $\M(\theta)$ parametrized with $\theta$:
	\begin{equation}
		\label{eq:model}
		\M(\theta): \left\{ \begin{array}{ll}
			x_{k+1}&= f(x_k,u_k;\theta) + w_k\\
			y_k& = h(x_k\red{}),%\pdfmargincomment[color=red]{We do not consider such systems!}
		\end{array} \right.
	\end{equation}
	where the system state, input, and observation at the $k^{\text{th}}$ time-step are denoted by $x_k, u_k, y_k$, respectively. The functions $f$ and $h$ specify, respectively, the parameterized state evolution of the system and the observation map. The additive noise is denoted by $w_k$, which is an independent, identically distributed \new{(i.i.d.)} noise sequence with distribution $w_k\sim p_w(\cdot)$.
\end{comment}
\Birgit{To obtain a bounded set $\Theta$, we use data-driven system identification, which}
%Data-driven system identification 
provides a solution to the following problem.
The true system $\M^\ast$ \pdfmargincomment{Birgit: Is it necessary to introduce this notation? Do you need it later on in the paper?}  to be identified is unknown and can only be observed through samples $(u,y)$, where the output measurements $y$ are undisturbed. We assume that the latent model $\M^\ast:=\M(\theta^\ast)$ can be described by \eqref{eq:model}, where the underlying true parametrization $\theta^\ast$ is unknown.
%For this, we excite the system with some input $u$. 
To infer the unknown parametrization, we collect data $\mathcal{D}$ from $\M^\ast$. For this, we sample a finite number of input-output sequences of the form
\begin{align}
	u^{(i)} = u^{(i)}_0,\ldots,u^{(i)}_{T-1},\qquad
	y^{(i)} = y^{(i)}_0,\ldots,y^{(i)}_{T-1}, \label{eq:data}
\end{align}
where $i=1,\ldots,N$ and $T$ are finite.
Based on $\mathcal{D}$, we estimate $\theta^\ast$ with an \emph{estimate} $\hat\theta$ and construct a \emph{confidence set} $\Theta$ which contains the true parameters $\theta^\ast$ with some given confidence $1-\alpha\in(0,1)$, i.e., $\P(\theta^\ast\in\Theta)\geq 1-\alpha$ (cf. Fig.~\ref{fig:confSetSketch}). We assume that $\hat\theta\in\Theta$. Note that there exists a wealth of data-driven identification methods providing accurate parameter estimates with the associated confidence sets. In Sec.~\ref{sec:establish_relation} we introduce two different methods for linear and nonlinear stochastic systems providing robust results, noting that they can be substituted to address a variety of different systems.
\begin{figure}[h]
	\centering
	\includegraphics[width=.7\columnwidth]{confSetSketch.png}
	\caption{The unknown true parameters $\theta^\ast$ are approximated with an estimate $\hat\theta$ and are robustly contained within a confidence set $\Theta$ with a confidence of $1-\alpha$. \red{Draft figure!}}
	\label{fig:confSetSketch}
\end{figure}

==> Gaussplot.tex <==
% !TEX root =  main.tex
%\begin{figure}[htp]
%%\pgfmathdeclarefunction{dnorm}{2}{%
%%	\pgfmathparse{1/(#2*sqrt(2*pi))*exp(-((x-#1)^2)/(2*#2^2))}%
%%}
%
%\begin{tikzpicture}
%	\begin{axis}[
%		domain=0:9,
%		samples=101,
%		height=5cm,
%		width=10cm
%		]
%		
%		% Fill aread under both curves, start stacking
%		\addplot [
%		fill=yellow,
%		draw=none,
%		domain=0:10,
%		stack plots=y
%		] {min(dnorm(4,1),dnorm(5,1)) } \closedcycle;
%	
%
%		% Draw curves
%		\addplot [thin, smooth, name path global=first] {dnorm(4,1)};
%		\addplot [thin, smooth, name path global=second] {dnorm(4,1)};
%
%	\end{axis}
%\end{tikzpicture}
%\caption{Computation of $\Wt$ given $\hat \Tr$ and $\Tr$. }\label{fig:Comp_W}
%\end{figure}

\begin{figure}[h]
\begin{tikzpicture} 
	\begin{axis}[samples=150,
		domain=-5:5,clip = false,
		xlabel={$\hat w$},
		zmin=0,
		zlabel={$p(dw)$},
		samples y=0, y dir=reverse, ylabel={$w$},
		area plot/.style={
			fill opacity=0.55,
			draw=none,
			fill=blue!70,
			mark=none,
			smooth
		}, ticks=none
		]
		% what
		\draw [black, densely dotted, style=thin] (axis cs: -5,0,0) -- (axis cs: -5,0,0.4);
		\draw [black, densely dotted, style=thin] (axis cs: -5,0,0) -- (axis cs: 0,0,0);
		\addplot3 [blue, mark=none, smooth, style=semithick, densely dashed] (-5,x,{min(dnorm(-1,1),dnorm(0,1)) });
		\addplot3 [black, mark=none, smooth, style=semithick, densely dashed]  (-5,x,{dnorm(0,1) });
		\addplot3 [black, mark=none, smooth, style=semithick, densely dashed]  (-5,x,{dnorm(-1,1) });
		\addplot3 [black, mark=none, smooth, style=semithick]  (-5,x,{min(dnorm(-1,1),dnorm(0,1)) });
		\draw [red, solid, style=semithick] (axis cs: -5,-1,0.4) -- (axis cs: -5,0,0.4);
		\draw [red, densely dotted, style=thin] (axis cs: -5,-1,0) -- (axis cs: -5,-1,0.4);
		\node (D) at (axis cs: -5,-1,0.4) [red, right] {$-\offset$};
		\addplot3 [area plot,fill=blue!30] (-5,x,{min(dnorm(-1,1),dnorm(0,1)) });
		% wbar
		\addplot3[blue, mark=none, smooth, style=semithick]  (x+1,x,{min(dnorm(0,1),dnorm(-1,1))});	
		\addplot3 [area plot] (x+1,x,{min(dnorm(0,1),dnorm(-1,1))});	
		\draw [black, densely dotted, style=thin] (axis cs: -5,-5,0) -- (axis cs: 5,5,0);
		% w
%		\draw (0,0) -- (6,0) -- (6,3) -- (0,3) -- cycle;
		\node (A) at (axis cs: 1,-5,0.4) [red, right] {$\offset$};
		\draw [red, solid, style=semithick] (axis cs: 1,-5,0.4) -- (axis cs: 0,-5,0.4);
		\draw [red, densely dotted, style=thin] (axis cs: 1,-5,0) -- (axis cs: 1,-5,0.4);
		\draw [black, densely dotted, style=thin] (axis cs: 0,-5,0) -- (axis cs: 0,-5,0.4);
		\draw [black, densely dotted, style=thin] (axis cs: 0,-5,0) -- (axis cs: 0,0,0);
		\addplot3 [blue, mark=none, smooth, style=semithick, densely dashed] (x,-5,{min(dnorm(1,1),dnorm(0,1)) });
		\addplot3 [black, mark=none, smooth, style=semithick, densely dashed]  (x,-5,{dnorm(1,1) });
		\addplot3 [black, mark=none, smooth, style=semithick, densely dashed]  (x,-5,{dnorm(0,1) });
		\addplot3 [black, mark=none, smooth, style=semithick]  (x,-5,{min(dnorm(1,1),dnorm(0,1)) });
		\addplot3 [area plot,fill=blue!30] (x,-5,{min(dnorm(1,1),dnorm(0,1)) });
		\node (B) at (axis cs: 7,-5,0.12) [black, right, rotate = 90] {$\hat p(d\hat w)$};
%		\node (C) at (axis cs: 0,6,0.2) [black, right, rotate = 30] {$t(d\xp)$};
		\node (C) at (axis cs: -1,0,0) [blue, rotate = -45]  {$\bar{{w}}(d\hat w\times dw)$};
	\end{axis}
\end{tikzpicture}
\caption{Two dimensional representation of the computation of the noise coupling $\bar{{w}}$ for two normally distributed noise distributions with offset $\offset$. Displayed is the noise coupling over the product space as well as its marginals, respectively. 
%	\Oliver{This figure might be unnecessary.} \Birgit{I agree.}
}
\label{fig:gaussplot}
\end{figure}

==> fullLTL.tex <==
% !TEX root =  main.tex
\section{Extensions of specification semantics}
\Oliver{Remove this section completely??}
Until now, we only addressed scLTL specifications. Now, we want to see whether we can extend the approach to more expressive semantics, e.g., full LTL properties.
\begin{remark}[Finite-trace LTL (LTL\textsubscript{f})]
	%[\bfseries Finite-trace full LTL (LTL\textsubscript{f})}]
	The method described in this work is naturally applicable for full LTL specifications over finite-traces (LTL\textsubscript{f}) using the native approach outlined in \cite{Wells2020ftLTL}.
	LTL\textsubscript{f} semantics are useful for formalizing finite-horizon planning problems.
	With the approach in \cite{Wells2020ftLTL} our results for SSRs can be extended to LTL\textsubscript{f} by first translating the LTL\textsubscript{f} formula to an equivalent intermediate first-order logic (FOL) formula \cite{DeGiacomo2013ftLTL2FOL} and subsequently generating a minimal DFA using, e.g., the tool MONA \cite{Henriksen1995MONA}.	
	Thereafter, the procedure remains the same, first constructing a product MDP and then solving the reachability problem (cf. \cite{haesaert2020robust}).
	
%	Note that LTL\textsubscript{f} is expressively equivalent to FOL \cite{Kamp1968FOL2ftLTLequivalence}.
%	Furthermore, interesting extensions to dealing with more expressive monadic second-order logics (MSO) as in linear dynamic logics (LDL\textsubscript{f}) are addressed in \cite{Zhu2019LTLf2DFA}.
\end{remark}

However, one of the main strengths of our approach resides in the possibility of addressing infinite horizon specifications. Naturally, this motivates extending the approach to infinite-trace LTL as well by, e.g., approximating the \red{Büchi} acceptance condition (repeated reachability) using the method outlined in \cite{kazemi2020fullLTL}. However, there are some major limitations as described in the following remark:
\newline

%From the results of the previous sections we have
%\begin{equation*}
%	\P\left(\Ca \times \M(\theta) \satisfies \psi_{scLTL} \right)\geq   p_{\psi_{scLTL}}, \quad  \forall \theta\in\Theta.
%\end{equation*}
%We now want to expand this to full LTL specifications, i.e.,
%\begin{equation*}
%	\P\left(\Ca \times \M(\theta) \satisfies \psi_{LTL} \right)\geq   p_{\psi_{LTL}}, \quad  \forall \theta\in\Theta.
%\end{equation*}
%
%From \cite{kazemi2020fullLTL} we have
%\begin{equation*}
%	p_l \leq \sup_{\Ca}\,\P\left(\Ca \times \M(\theta) \satisfies \psi_{LTL} \right) \leq p_u, \quad  \forall \theta\in\Theta,
%\end{equation*}
%where the upper and lower bounds are given by
%\begin{align*}
%	p_u &:= \sup_{\boldsymbol{\mu}}\,\P\left(\boldsymbol{\mu} \times \left(\M(\theta) \times \tilde{\mathcal{A}}_\psi\right)_\zeta \satisfies \Event\phi \right)\text{, and}\\
%	p_l &:= 1-\sup_{\boldsymbol{\mu}}\,\P\left(\boldsymbol{\mu} \times \left(\M(\theta) \times \tilde{\mathcal{A}}_{\notltl\psi}\right)_\zeta \satisfies \Event\phi \right).
%\end{align*}
%Here, $\Ca$ is a finite-memory control strategy \Oliver{(Check whether definition in Sec.~\ref{sec:MDPs} is valid for this (freedom to use LDBA instead of DFA?!))}, whereas $\boldsymbol{\mu}$ is a Markov policy. Furthermore, $\tilde{\mathcal{A}}_\psi$ is a LDBA for specification $\psi$.

\Oliver{(I just added the following part to show the theory behind the computations regarding fullLTL. The results are summarized in Rem.~\ref{rem:fullLTL})}

\color{gray}
As in \cite{haesaert2020robust} we want to compute the following. For the bounded horizon $N$ and Markov policy $\boldsymbol{\mu}$ define value functions $V^{\boldsymbol{\mu}}_k:\X\times Q\rightarrow[0,1]$, $k\in[0,N]$, as the probability that the sink state $\phi\in\X\times Q$ is reached within $k$ time steps starting from the product state $(x,q)$ at time $N-k$:
\begin{align*}
	V^{\boldsymbol{\mu}}_k (x, q) := \mathbb{E}\left[ \max_{N-k<t\leq N} \1_\phi(x_t, q_t) \given x_{N-k}=x, q_{N-k}=q \right] 
\end{align*}
We have with $V^{\boldsymbol{\mu}}_0 = 0$ and compute recursively via 
\begin{align*}
	V^{\boldsymbol{\mu}}_{k+1} (x, q) = \mathbf T^{\mu_l}(V^{\boldsymbol{\mu}}_k (x, q)),\quad k\in[0,N-1]
\end{align*}
with $l:=N-(k+1)$ and the Bellman operator
\begin{align}
	\begin{split}
		\mathbf T^{\mu}&(V)(\hat x,q) := \int_{(\X\times Q)\cup\phi}\!\!\!\max\left\lbrace \1_\phi(x',q'), V(x',q') \right\rbrace\\
		&\hspace{1cm}\times \tilde{\mathbf{t}}(dx'\times\left\lbrace q'\right\rbrace | (x, q), \mu(x, q) ),
	\end{split}\label{eq:bellman_operator}
\end{align}
where the augmented kernel $\tilde{\mathbf{t}}:((\X\times Q)\cup\phi)\times\A\times\mathcal B((\X\times Q)\cup\phi)\rightarrow[0,1]$ is defined as follows:
\begin{align}
	\begin{split}
		\tilde{\mathbf{t}}(\phi | \phi, \mu)&=1\\
		\tilde{\mathbf{t}}(\phi | (x, q), \mu)&=(1-\xi)\1_B(x,q)\\
		\tilde{\mathbf{t}}(A | (x, q), \mu)&=[1-(1-\xi)\1_B(x,q)]\bar{\mathbf{t}}(A | x,q,\mu),
	\end{split}\label{eq:aug_kernel}
\end{align}
for all $A\in B(\X\times Q)$, $(x,q)\in\X\times Q$, and for any accepting states $(x,q)\in B$.

\Oliver{(Omitting two propositions about the bounded reachability probability and the optimal bounded reachability probability as in \cite{haesaert2020robust}.)}

We can split the integral in the Bellman operator in \eqref{eq:bellman_operator} to obtain
\begin{align*}
	\mathbf T^{\mu}&(V)(\hat x,q) := \int_{\X\times Q}\!\!\!V(x',q')\times \tilde{\mathbf{t}}(dx'\times\left\lbrace q'\right\rbrace | (x, q), \mu )\\
	&\hspace{1cm}+\textcolor{purple}{\int_{\phi}\tilde{\mathbf{t}}(dx'\times\left\lbrace q'\right\rbrace | (x, q), \mu )},
\end{align*}
and with \eqref{eq:aug_kernel}
\begin{align*}
	&\mathbf T^{\mu}(V)(\hat x,q) :=\\
	&\hspace{0.5cm}\begin{cases}
		1, \quad \text{for $(x,q)=\phi$,}\\
		[1-(1-\xi)\1_B(x,q)] \int_{\X\times Q}V(x',q') \times\bar{\mathbf{t}}(dx'\times\left\lbrace q'\right\rbrace | x,q,\mu)\\
		\hspace{0.5cm} + \textcolor{purple}{(1-\xi)\1_B(x,q)},\quad\text{otherwise.}
	\end{cases}
\end{align*}

For the $\delta$-robust operator $\mathbf T_{\delta}^{\mu}(V)(\hat x,q) :=\Lim\Big( \mathbf T^{\mu}(V)(\hat x,q) -\delta\Big)$ as defined in \cite{haesaert2020robust} we get
\begin{align*}
	&\mathbf T_{\delta}^{\mu}(V)(\hat x,q) :=\\
	&\hspace{0.5cm}\begin{cases}
		1, \quad \text{for $(x,q)=\phi$,}\\
		\Lim\Big([1-(1-\xi)\1_B(x,q)]\int_{\X\times Q} V(x',q') \times\bar{\mathbf{t}}(dx'\times\left\lbrace q'\right\rbrace | x,q,\mu)\\
		\hspace{0.5cm} + \textcolor{purple}{(1-\xi)\1_B(x,q)} -\delta\Big),\quad\text{otherwise,}
	\end{cases}
\end{align*}
where the subtraction of $\delta$ was omitted for $(x,q)=\phi$ because $\phi$ is a sink state.

Taking the worst-case automaton transition with right to an $\varepsilon$-ball around $\xh{}'$ yields the $(\varepsilon,\delta)$-optimal operator
\begin{align*}
	&\mathbf T_{\varepsilon,\delta}^{\mu}(V)(\hat x,q) :=\\
	&\hspace{0.5cm}\begin{cases}
		1, \quad \text{for $(x,q)=\phi$,}\\
		\Lim\Big([1-(1-\xi)\1_B(x,q)]\int_{\hat\X} \min_{q'\in \bar\trans(q,\hat x')} \left\lbrace V(\hat x',q')\right\rbrace\\
		\hspace{0.5cm}  \times {\mathbf{t}}(dx' | x,q,\mu)
		+ \textcolor{purple}{(1-\xi)\1_B(x,q)} -\delta\Big),\quad\text{otherwise.}
	\end{cases}
\end{align*}

\color{blue!70!black}
\begin{remark}[Full LTL]\label{rem:fullLTL}
	There are two main limitations for extending the robust controller synthesis as in Prop.~\ref{prop:delepsreach_infty} to infinite-trace LTL. 
	Both factors otherwise lead to a zero-valued lower bound on the satisfaction probability.
	Firstly, for unbounded support, in every step there exists a non-zero probability of transitioning outside the specified state-space region. Since approximating the \red{Büchi} condition using the method from \cite{kazemi2020fullLTL} entails only accepting infinite words, this leads to a zero-valued lower bound as well. Obviously, this can be overcome by choosing a bounded support.
	Secondly, and the more limiting factor, approximating the \red{Büchi} acceptance condition with a non-zero $\delta$ leads to trivial results, therefore necessitating an SSR with $\delta=0$. \Oliver{Wrote proof that this would mean that $\Wt$ cannot be a sub-probability measure and cannot compensate parameter uncertainty.}
\end{remark}

This motivates us to look at bounded disturbances, i.e., bounded transition probabilities (in practice often the case). \Oliver{Might work well to put the section about bounded support here.}


\begin{comment}
We get 
\begin{align*}
	\mathbf T_{}^{\mu} (V)(\hat x,q)\!:=\!
	\begin{cases}
		1 \text{, for $(\hat x,q)=\phi$}\\
		(1-\xi)+\xi \int_{\Xh}V(\hat x',q') \times \bar\trans(q'|q,\hat x')\times \Trh(d \hat x'| \hat x,\mu) \text{, for $(\hat x,q)\in F$}\\
		\int_{\Xh}V(\hat x',q') \times \bar\trans(q'|q,\hat x')\times \Trh(d \hat x'| \hat x,\mu) \text{, otherwise}
	\end{cases}
\end{align*}
with $\bar\trans(q,\hat x'):=\{\trans(q,\alpha)\mbox{ with }\alpha \in\Lab(B_\varepsilon( \hat h (\hat x')))\}$.
%Since the integral term is upper bounded by one, the term in the second case is always greater or equal to the third one and hence we can write
%\begin{align*}
%	&\mathbf T_{}^{\mu} (V)(\hat x,q)\!:=\!\\
%	&\int_{\Xh} \max\left\{\1_{\phi}(\hat x, q), \1_{F}(\hat x, q)(1-\xi)+\xi \int_{\Xh}V(\hat x',q') \times \Trh(d\hat x'|\hat x,\mu) \times \bar\trans(q'|q,\hat x'), \int_{\Xh}V(\hat x',q') \times \Trh(d\hat x'|\hat x,\mu) \times \bar\trans(q'|q,\hat x')\right\}
%\end{align*}
We define the $\delta$-robust operator
\begin{align*}
	\mathbf T_{\delta}^{\mu} (V)(\hat x,q)\!:=\!\Lim\left(
	\begin{cases}
		1-\delta \text{, for $(\hat x,q)=\phi$}\\
		(1-\xi)+\xi \int_{\Xh}V(\hat x',q') \times \bar\trans(q'|q,\hat x')\times \Trh(d \hat x'| \hat x,\mu)-\delta \text{, for $(\hat x,q)\in F$}\\
		\int_{\Xh}V(\hat x',q') \times \bar\trans(q'|q,\hat x')\times \Trh(d \hat x'| \hat x,\mu)-\delta \text{, otherwise}
	\end{cases}\right) 
\end{align*}
and the optimal $\delta$-robust operator
\begin{align*}
	\mathbf T_{\delta}^{\ast} (V)(\hat x,q)\!:=\!\sup_{\mu}\Lim\left(
	\begin{cases}
		1-\delta \text{, for $(\hat x,q)=\phi$}\\
		(1-\xi)+\xi \int_{\Xh}V(\hat x',q') \times \bar\trans(q'|q,\hat x')\times \Trh(d \hat x'| \hat x,\mu)-\delta \text{, for $(\hat x,q)\in F$}\\
		\int_{\Xh}V(\hat x',q') \times \bar\trans(q'|q,\hat x')\times \Trh(d \hat x'| \hat x,\mu)-\delta \text{, otherwise}
	\end{cases}\right) 
\end{align*}

For the optimal $(\varepsilon,\delta)$-robust operator we get
\begin{align*}
	\notag \textstyle \mathbf T_{\eps,\delta}^{\ast} (V)(\hat x,q)\!:=\!
	\sup_{\mu}\Lim\left( \!\!\int_{\hat\X} \min_{q'\in \bar\trans(q,\hat x')}\!\!\
	\begin{cases}
		1-\delta \text{, for $(\hat x,q)=\phi$}\\
		(1-\xi)+\xi \int_{\Xh}V(\hat x',q') \times \Trh(d\hat x'|\hat x,\mu)-\delta \text{, for $(\hat x,q)\in F$}\\
		\int_{\Xh}V(\hat x',q') \times \Trh(d\hat x'|\hat x,\mu)-\delta \text{, otherwise}
	\end{cases}\right)
\end{align*}
which takes the worst-case location $q'$ considering an $\varepsilon$-ball around the systems output $\hat h (\hat x')$ as described earlier.
\color{black}
\end{comment}

%\color{red}
%\begin{align*}
%	\notag \textstyle \mathbf T_{\eps,\delta}^{\ast} (V)(\hat x,q)\!:=\!
%	\sup_{\mu}\Lim\left( \!\!\int_{\hat\X} \min_{q'\in \bar\trans(q,\hat x')}\!\!\
%	\begin{cases}
%		1-\delta \text{, for $(\hat x,q)=\phi$}\\
%		(1-\xi)+\xi \int_{\Xh}V(\hat x',q') \times \Trh(d\hat x'|\hat x,\mu)-\delta \text{, for $(\hat x,q)\in F$}\\
%		\int_{\Xh}V(\hat x',q') \times \Trh(d\hat x'|\hat x,\mu)-\delta \text{, otherwise}
%	\end{cases}\right)
%\end{align*}
%wrong!!




==> new_case_studies.tex <==
% !TEX root = main.tex
\subsection{Linear system with complex specification}
%\red{Need to update all results to without measurement noise!}

Consider two uncertain linear systems, i.e., Eqs.~\eqref{eq:sysDataGenNonlin}-\eqref{eq:sysInfNonlin} with 
$f(x_k, u_k) = \left[ x_k,u_k \right]\T$, $h(x_k)=\hat h(x_k)=x_k$,
%, where $A:=[\theta_1,0.3;0.2,0.7]$, $B:=[\theta_2,0;0,1.4]$, $\sigma_w^2:=1$, and $C:=[1,0;0,1]$, describing an agent translating in a 2D space.
and $\sigma_w^2:=1$, describing an agent translating in a 2D space.
% and $v_k\sim \mathcal N(0,\sqrt{0.1}I)$
Define the state space $\X = [-6,6]^2$, input space $\U = [-1,1]\red{?}$, and output space $\Y = \X$.
The goal is to compute a controller for a package delivery problem.
For this, the controller should navigate the agent to pick up a parcel at region $P_1$ and deliver it to target region $P_3$. If the agent passes the avoid region $P_2$ on its path, it loses the package and must pick up a new one (at $P_1$). This desired behavior is captured by the specification $\psi = \Event(P_1 \andltl (\notltl P_2 \Until P_3))$. Note that the corresponding DFA contains a backward loop from location $q_1$ (cf. Fig~\ref{fig:dfa_delivery}) and is hence not not expressible as a reach-avoid specification over the state space only. 
Here, we consider
$P_1 =[3,6]\times[-2.5,1]$, $P_2 =[-1,1]\times[-4,3]$,
and $P_3 =[-6,-3]\times[-6,-3]$.
\begin{figure}
	\centering
	\begin{tikzpicture}
		\node[state, initial] (q0) {$q_0$};
		\node[state, right of=q0, xshift=1.5cm] (q1) {$q_1$};
		\node[state, accepting, right of=q1, xshift=1.5cm] (q2) {$q_F$};
		\path[-stealth]
		(q0) edge[loop above] node{$\neg P_1$} (q0)
		(q0) edge[above] node{$ P_1$} (q1)
		(q1) edge[loop above] node{$\neg P_2 \wedge\neg P_3$} (q1)
		(q1) edge[bend left, below] node{$P_2$} (q0)
		(q1) edge[above] node{$P_3 \wedge\neg P_2$} (q2)
		(q2) edge[loop above] node{$1$} (q2)
		;
	\end{tikzpicture}
	\caption{DFA corresponding to the package delivery problem.}
	\label{fig:dfa_delivery}
\end{figure}

For estimating the parameters, we sample $N=10^4,10^5,10^6$ data points from the true system with parametrization $\theta^\ast = \left[0.6,0.3,0,0;0.2,0.7,0,0;0,0,1.2,0;0,0,0,1.4\right]$ using an excitation $u\sim\mathcal{N}(0, \red{?})$.
Using Bayesian linear regression, we obtain an estimate $\hat\theta$ and a confidence set $\Theta$
(displayed for $(\theta_{11}, \theta_{33})$ in Fig.~\ref{fig:confSetDelivery})
for a lower confidence bound of 0.9 as outlined in Sec.~\ref{sec:BLR}.
Note that the confidence set contracts for increasing amounts of data.
We select $\Mh=\M(\hat\theta)$ to be the nominal model and get $\eps_1=0$.
A state-input-dependent $\delta_1$ is computed using Eq.~\eqref{eq:delta_ddnonlinear}, displayed in Fig.~\ref{fig:delta1ANDsatProb_Delivery}.
Note that $\delta_1$ grows rapidly for states away from the central region, thus a global upper bound on $\delta_1$ would result in poor satisfaction probabilities.
\color{black}
We compute a second abstract model $\Mt$ by discretizing the space of $\Mh$. Then, we use the results of \cite{haesaert2020robust} to get ${\Mt}\preceq^{\delta_2}_{\eps_2}\Mh$ with $\eps_2=0.016$ and $\delta_2=0.016$. Thus, we have $\Mt\preceq^{\delta}_{\eps}\M(\theta)$ with $\delta = \delta_1+\delta_2$ and $\eps = \eps_1 + \eps_2$.
The probability of satisfying the specification with this $\eps$ and $\delta$ is computed based on Thm.~\ref{prop:delepsreach_infty} and is depicted in Fig.~\ref{fig:delta1ANDsatProb_Delivery} as a function of the initial state of $\M$. 
%\new{Results for varying amounts of data are given in Tbl.~\ref{tbl:resultsDelivery}.}
An exemplary trajectory of the controlled system initialized at $x_0=[-5, -5]$ and run 
until satisfaction
%for $N=60\red{?!}$\pdfmargincomment{Two uses for $N$!} time steps 
is shown in Fig.~\ref{fig:delivery_Sim}. This emphasizes the capability of the proposed approach of being able to synthesize controllers guaranteeing satisfaction of complex temporal logic specifications over infinite-horizon runs, unique in the literature.
\begin{figure}
	\centering
	\includegraphics[width=\columnwidth]{confSetDelivery_1e3456.eps}
	\caption{\red{Will be updated. Will add $\hat\theta\approx\theta^\ast$ and $N$ labels.} Contracting confidence set $\Theta$ for $N=10^3,10^4,10^5,10^6$ data sequences with an associated lower confidence bound of $0.9$.}
	\label{fig:confSetDelivery}
\end{figure}

%\begin{figure}
%	\centering
%	\includegraphics[width=\columnwidth]{resultsDelivery_1e4.eps}\\
%	\vspace{0.1cm}
%	\includegraphics[width=\columnwidth]{resultsDelivery_1e5.eps}\\
%	\vspace{0.1cm}
%	\includegraphics[width=\columnwidth]{resultsDelivery_1e6.eps}
%	\caption{\red{Draft. Will be updated.} Lower bound on the satisfaction probability and values of $\delta_1$ as a functions of the initial state for $N=10^4,10^5,10^6$ (top to bottom) for the package delivery case study with a confidence of $1-\alpha=0.9$.}
%	\label{fig:delta1ANDsatProb_Delivery}
%\end{figure}
\begin{figure*}
	\centering
	\includegraphics[width=.32\textwidth]{resultsDelivery_1e4.eps}
	\hfill
	\includegraphics[width=.32\textwidth]{resultsDelivery_1e5.eps}
	\hfill
	\includegraphics[width=.32\textwidth]{resultsDelivery_1e6.eps}
	\caption{\red{Draft. Will be updated.} Lower bound on the satisfaction probability and values of $\delta_1$ as a functions of the initial state for $N=10^4,10^5,10^6$ (top to bottom) for the package delivery case study with a confidence of $1-\alpha=0.9$.}
	\label{fig:delta1ANDsatProb_Delivery}
\end{figure*}

\begin{figure}
	\centering
	\includegraphics[width=\columnwidth]{PckDelivery_SimMulti.eps}
	\caption{\red{Will be updated.} Two exemplary satisfying trajectories for the package delivery study. Note that the magenta agent takes loses a parcel in $p_2$ and has to take an additional loop. (N=?)}
	\label{fig:delivery_Sim}
\end{figure}

%\subsection{Data-driven linear system}
%
%Real system is subject to drag and mass deviation impacting the change of velocities:
%\begin{equation*}
%	\begin{bmatrix}x_1^+\\v_1^+\\d^+\end{bmatrix} = \begin{bmatrix}1&\tau&0\\0&\theta_1&0\\0&\tau&1\end{bmatrix}\begin{bmatrix}x_1\\v_1\\d\end{bmatrix}
%	+ \begin{bmatrix}0\\\tau\theta_3\\0\end{bmatrix}u_1
%	+\begin{bmatrix}0\\1\\0\end{bmatrix}w_1
%	\red{+\begin{bmatrix}0\\0\\-\tau\end{bmatrix}v_2},
%\end{equation*}
%where the control input $u$ is the acceleration of the car and $y=x$.
%
%Hence we get
%\begin{align*}
%	&G(\theta) = C\begin{bmatrix} B(\theta) & AB(\theta) & \ldots & [A(\theta)]^{T-2}B(\theta) \end{bmatrix} \in \R^{p\times m(T-1)}\\
%	&= \begin{bmatrix} 
%		0 & \tau^2\theta_3 & \tau^2\theta_3+\tau^2\theta_1\theta_3 
%%		& \tau^2\theta_3+\tau^2\theta_1\theta_3+\tau^2\theta_1^2\theta_3 
%		& \ldots \\
%		\tau\theta_3 & \tau\theta_1\theta_3 & \tau\theta_1^2\theta_3 
%%		& \tau\theta_1^3\theta_3 
%		& \ldots \\
%		0 & \tau^2\theta_3 & \tau^2\theta_1\theta_3+\tau^2\theta_3 
%%		& \tau^2\theta_1^2\theta_3+\tau^2\theta_1\theta_3+\tau^2\theta_3 
%		& \ldots
%	\end{bmatrix}.
%\end{align*}
%\Oliver{Could also just look at G over first two rows/state variables.}
%With unknown true values $\theta^\ast_1=0.9, \theta^\ast_2=0.7$.
%With nominal values $\theta_1=1, \theta_2=1$.
%Identified estimate $\hat\theta$ from first and second column of $G_(\theta)$. Because the last state variable is decoupled from the external input we can not use it for parameter estimation.
%
%The confidence set can be derived as follows (omitting index for subsystem): \Oliver{First two states only.}
%\begin{align*}
%	\Phi &\geq \norm{\hat G-G(\theta)} \\
%	&= \norm{C[\hat B-B(\theta), \hat B\hat A-B(\theta)A(\theta),\ldots]}\\
%	&= \norm{\begin{bmatrix} 
%			0 & \tau^2(\hat\theta_3-\theta_3) & \ldots \\
%			\tau(\hat\theta_3-\theta_3) & \tau(\hat\theta_1\hat\theta_3-\theta_1\theta_3) & \ldots
%	\end{bmatrix}}
%\end{align*}
%%Therefore, we can write the confidence set of subsystem one as a function of the LS estimate:
%%\begin{equation*}
%%	\Theta(\hat\theta) := \left\lbrace (\theta_1,\theta_3)\in\R^{2\mathfrak{p}}\given\max_{\abs{\lambda_1+\lambda_2}=1}\abs{\lambda_1a(\theta,\hat\theta) + \lambda_2b(\theta,\hat\theta)}\leq\Phi \right\rbrace.
%%\end{equation*}
%
%\color{red}
%Here, we only use two columns since $T=3$.
%For $\delta$ we get the following optimization problem:
%\begin{align*}
%	\delta(z, \hat\theta) = &\max_{\theta} \left\lbrace 1-2\cdot\cdf{-\frac{1}{2}\norm{\begin{bmatrix}
%		x_{k,1}+\tau x_{k,2} \\ \theta_1 x_{k,2} +\tau\theta_2 u_k
% 	\end{bmatrix}}}\right\rbrace\\
%	&\text{s.t.}\quad \norm{\begin{bmatrix} 
%			0 & \tau^2(\hat\theta_3-\theta_3) \\
%			\tau(\hat\theta_3-\theta_3) & \tau(\hat\theta_1\hat\theta_3-\theta_1\theta_3)
%	\end{bmatrix}}\leq\Phi
%\end{align*}



==> nonlinear_apprx.tex <==
% !TEX root =  main.tex
Consider two bounds. One bound on the step by step deviation that can be caused by the unknown parameter, and one deviation that is caused by state discrepancies between the two models. 
Let us assume that for the former, we can bound it as
\begin{align}
\|	f(x_k, u_k;\theta)-f(x_k, u_k;\theta_0)\|\leq d.
\end{align}

We can rewrite the original model as follows:
\begin{align*}
	x_{k+1} &=\underbrace{f(x_k, u_k;\theta_0)}_{nominal dynamics} + \underbrace{ f(x_k, u_k;\theta)-f(x_k, u_k;\theta_0)+w_k}_{disturbance}.
\end{align*}

We can now start relating the stochastic models by coupling over a subset where the disturbances are equal, that is, we search for a sub-probability coupling $\bar{\mathbf{w}}$ for which $\support(\bar{\mathbf{w}})\subset \{f(x_k, u_k;\theta)-f(x_k, u_k;\theta_0)+w_k= \hat w_k\}$. 

This leads to a sub-probability kernel $\Wt$ that is similar to the kernel \eqref{eq:ex_v} in   Example \ref{ex:lineartheta}, and that is hence similarly based on a sub-probability coupling \eqref{eq:ex_w}. 
If we look at the behaviour of the two stochastic systems constrained to $  \{f(x_k, u_k;\theta)-f(x_k, u_k;\theta_0)+w_k= \hat w_k\}$, we have that  
\begin{align*} 
		\hat x_{k+1} &=   f(\hat x_{k},\hat u_k; \theta_0)+  \hat  w_k\\
		x_{k+1} &=f(x_k, u_k;\theta_0) + \underbrace{ f(x_k, u_k;\theta)-f(x_k, u_k;\theta_0)+w_k}_{=\hat w_k}.
\end{align*}
Furthermore, the error dynamics $\Delta x_k:= 	x_{k}-\hat x_k $ evolve as
 \begin{align*} 
\Delta	x_{k+1} &=f(x_k, u_k;\theta_0) -   f(\hat x_{k},\hat u_k; \theta_0).
\end{align*}
As an update relation we get
\begin{equation}
	\hat x_{k+1} = x_{k+1} + f(\hat x_{k},\hat u_k; \theta_0) - f(x_k, u_k;\theta_0).
\end{equation}

==> paramEst.tex <==
% !TEX root =  main.tex
\color{blue!70!black}
\subsection{Data-driven simulation relations for linear systems}
In this subsection, we show how the approach for realizing simulation relations for linear systems (Sec.~\ref{sec:simrel_affine}) can be combined with robust parameter estimation to both address large scale and conservatism. For this, we gather observational data from the true model and learn the uncertain set $\Theta$ in a data-driven manner. We showcase this procedure for a linear stochastic system, noting that any method able to provide robust confidence sets of the uncertain parameter can be deployed in its place. Therefore, in general, a plethora of systems can be addressed.

Consider the following uncertain single-input single-output (SISO) system in its input-output form
\begin{equation*}
	y_k = G(\theta)u_k + \tilde w_k,
\end{equation*}
with a transfer function
\begin{equation*}
	G(\theta) = \dfrac{b_m z^{-m}+b_{m-1} z^{-m+1}+\ldots+b_1z^{-1}}{z^{-n}+a_{n-1}z^{-n+1}+\ldots+a_1z^{-1}+1},
\end{equation*}
strictly proper, i.e., $n>m$. Here, $z^{-1}$ denotes the backward shift operator.
%\red{We set $a_0=1$ and $b_0=0$.} 
This system can be equivalently written in its canonical state-space representation as
\begin{align*}
	\M(\theta): \left\{ \begin{array}{ll}
		x_{k+1}&=Ax_k+bu_k+w_k\\
		y_k &= c\T x_k,
	\end{array} \right.
\end{align*}
where
\begin{align*}
	A &= \begin{bmatrix}0&1&&\\\vdots&&\ddots&\\0&&&1\\-1&-a_1&\hdots&-a_{n-1}\end{bmatrix}, \quad 
	b = \begin{bmatrix}0\\\vdots\\0\\1\end{bmatrix}, \\
	c\T &= \begin{bmatrix}0&b_1&\hdots&b_m&0&\hdots&0\end{bmatrix}.
\end{align*}
%\begin{align*}
%	\M(\theta): \left\{ \begin{array}{ll}
	%		x_{k+1}&=\underbrace{
		%%			\begin{bmatrix}0&1&0&\hdots&0\\0&0&1&\ddots&\vdots\\\vdots&&&\ddots&0\\0&0&\hdots&0&1\\-a_0&\hdots&\hdots&\hdots&-a_{n-1}\end{bmatrix}
		%			\begin{bmatrix}0&1&&\\\vdots&&\ddots&\\0&&&1\\-a_0&\hdots&\hdots&-a_{n-1}\end{bmatrix}
		%		}_{A}x_k
	%		+\underbrace{\begin{bmatrix}0\\\vdots\\0\\1\end{bmatrix}}_{b}u_k+w_k\\
	%		y_k &= \underbrace{\begin{bmatrix}b_0-a_0b_n&\hdots&b_m\end{bmatrix}}_{c\T}x_k.
	%	\end{array} \right.
%\end{align*}
%with 
%\begin{align*}
%	A &= && B =\\
%	C &= && D =
%\end{align*}
%\Oliver{$w_k$ might be wrong.}
Without loss of generality, we assume that $w_k\sim\mathcal N(0,1)$.
The uncertain parameter is defined as $\theta:=[???]\T\in\Theta$.
The true unknown system is $\M(\theta^\ast)$ with some $\theta^\ast\in\Theta$.

\Oliver{Index shift from here:}
Let $u_{k}$, $k\in\{1-n-m,\ldots,N\}$ be an i.i.d. sequence of random variables symmetrically distributed around 0.
Assume that we acquired a finite number of input-output data $\mathcal{D}_N$ from $\M(\theta^\ast)$, namely
\begin{equation*}
	\mathcal{D}_N:=\left\lbrace (y_{k-1}, u_{k-1}, y_k) \right\rbrace,\quad k\in\{0,\ldots,N+1\},
\end{equation*}
where $N$ denotes the finite number of samples. \Oliver{Shift index and re-define $N$.} Note that we assume full-state observability.

Based on this data, we produce a robust estimate $\hat\theta_N\in\hat\Theta_N$ of the true uncertain parameter $\theta^\ast$ with an associated confidence region $\hat\Theta_N\subset\Theta$ that contains $\theta^\ast$ with a given probability $\mathbb{P}(\theta^\ast\in\hat\Theta)$.
For this, we employ the extended version of the \emph{leave-out sign-dominated correlation regions} (LSCR) method introduced in \cite{campi2010Confidence}.
One major advantage of this method is that it is not limited to Gaussian noise and works with bounded and unbounded support.
We summarize the main results of \cite{campi2010Confidence} in the following.
\Oliver{Consider changing the notation of the nominal $\hat\theta$ throughout the paper.}

%\Oliver{Outline following procedure briefly.}
The extended LSCR method relies on the fact that the prediction errors between the abstract system $\Mh(\hat\theta)$ and the true system $\M(\theta^\ast)$ should be uncorrelated with any past data. Its four step procedure involves computing the predictions of the abstract model using an initial guess of the parameters; computing the corresponding prediction errors; generating random binary strings; and constructing the confidence region based on correlational results.
%\Oliver{Note which assumptions hold or are imposed}
\subsubsection{Compute predictions} 
We start by making predictions as functions of $\theta$, namely
\begin{equation*}
	\hat y_k(\theta) = G(\theta)u_k=\psi\T_k\theta,
\end{equation*}
where $\psi\T_k := [-y_{k-1},\ldots,-y_{k-n};u_{k-1},\ldots,u_{k-m}]$.

\subsubsection{Compute prediction errors} 
The prediction error $\epsilon_k(\theta)$ for some $\theta\in\Theta$ can hence be written as
\begin{equation*}
	\epsilon_k(\theta) = y_k-\hat y_k(\theta)= y_k-\psi\T_k\theta.
\end{equation*}

\subsubsection{Generate random binary strings} 
Select an integer $M$ and construct $M$ unique stochastic binary strings of length $N$, including the zero string, as follows
\begin{align*}
	h_{0,1},\ldots,h_{0,N}:=0,\ldots,0\\
	h_{i,k}\sim p_b,&&k\in\{1,\ldots,N\},
\end{align*}
where $p_b$ is the binary probability distribution taking values of 0 or 1 with a probability of 0.5, each. Note that unique means $\forall i,j\in\{1,\ldots,N\}: h_{i,0},\ldots,h_{i,N}\neq h_{j,0},\ldots,h_{j,N}$ for $i\neq j$.

\subsubsection{Define correlation functions} 
%Form a vector
%\begin{equation*}
%	\xi_k=\begin{bmatrix}u_{k-1},\ldots,u_{k-n}\end{bmatrix}\T,\quad k=1,\ldots,N.
%\end{equation*}
Using the previously computed prediction errors $\epsilon_k(\theta)$, as functions of $\theta$, we define the following $2M$ functions
\begin{align}
	g_{i,j}(\theta)&:=\sum_{k=1}^{N} h_{i,k}u_{k-j}\epsilon_{k,j}(\theta),\label{eq:fun_g}
\end{align}
with $i\in\{0,\ldots,M-1\}$ and $j\in\{1,\ldots,n\}$ and where $\epsilon_{k}(\theta)=[\epsilon_{k,1}(\theta),\ldots,\epsilon_{k,n}(\theta)]\T$.

%\subsubsection{Construct confidence set} 
We construct the confidence set $\hat\Theta_N$ using the procedure outlined in \cite{campi2010Confidence}, Sec.~III. 
Based on \cite{campi2010Confidence}, Cor.~2, we can assign a confidence to $\hat\Theta_N$ as given in the following proposition.

\begin{proposition}[Confidence set]
	Assume that $\forall j\in\{1,\ldots,n\},i\neq 0:\,\mathbb{P}(g_{i,j}(\theta^\ast)=0)=0$.
	Choose an integer $q\in[1,M/(2n)]$ and sets $\hat{\Theta}_{N,1},\ldots,\hat{\Theta}_{N,n}\in\Theta$ such that
	%	\begin{itemize}
		%		\item[a)]
		for at least $q$ of $M$ functions $g_{i,j}(\theta)$ as defined in \eqref{eq:fun_g} we have $\forall j\in\{1,\ldots,n\}:\,g_{i,j}(\theta)>0$.
		%		\item[b)] for at least $q$ of $M$ functions $g_{i,2}(\theta)$ as defined in \eqref{eq:fun_g} we have $g_{i,2}(\theta)>0$.
		%	\end{itemize}
	Then, we find a confidence set
	\begin{equation}
		\hat\Theta=\bigcap_{l=1}^{n}  \hat{\Theta}_{N,l}\label{eq:confset}
	\end{equation}
	with a lower bound on the confidence that it contains the true uncertain parameter $\theta^\ast$, namely
	\begin{equation*}
		\mathbb{P}(\theta^\ast\in\hat\Theta) \geq 1-\frac{2nq}{M}.
	\end{equation*}
\end{proposition}
\Oliver{Remark about validity of assumption raised.}

\begin{proposition}[Robust parameter estimate]
	We obtain a robust parameter estimate
	\[\hat\theta_N=\{\exists\theta\in\Theta\given\sum_{k=1}^{N}\sum_{j=1}^{n}u_{k-j}\epsilon_{k,j}(\theta)=0\},\]
	that is guaranteed to lie in $\hat\Theta$ in \eqref{eq:confset}.
\end{proposition}

\color{gray}
\hrule
%For the sake of simplicity, consider the following uncertain linear single-input single-output (SISO) system
%\begin{equation*}
%	\M(\theta): \left\{ \begin{array}{ll}
	%		x_{k+1} &= \theta_1x_{k}+ \theta_2 u_k+ w_k\\
	%		y_k &= x_k,
	%	\end{array} \right.
%\end{equation*}
%with an uncertain parameter $\theta:=[\theta_1,\theta_2]\T\in\Theta$.
%%, and the nominal model
%%\begin{align*}
%%	\Mh: \left\{ \begin{array}{ll}
	%%		\hat x_{k+1} &= \hat a \hat x_{k}+ \hat b \hat u_k+\hat w_k\\
	%%		\hat y_k &= \hat x_k.
	%%	\end{array} \right.
%%\end{align*}
%Without loss of generality, we assume that $w_k\sim\mathcal N(0,1)$.
%The true unknown system is $\M(\theta^\ast)$ with some $\theta^\ast\in\Theta$.
%Let $u_{k-1}$, $k\in\{0,\ldots,N+1\}$ be an i.i.d. sequence of random variables symmetrically distributed around 0.
%Assume that we acquired a finite number of input-output data $\mathcal{D}_N$ from $\M(\theta^\ast)$, namely
%\begin{equation*}
%	\mathcal{D}_N:=\left\lbrace (y_{k-1}, u_{k-1}, y_k) \right\rbrace,\quad k\in\{0,\ldots,N+1\},
%\end{equation*}
%where $N$ denotes the finite number of samples. Note that we assume full-state observability.
%
%Based on this data, we produce a robust estimate $\hat\theta_N\in\hat\Theta_N$ of the true uncertain parameter $\theta^\ast$ with an associated confidence region $\hat\Theta_N\subset\Theta$ that contains $\theta^\ast$ with a given probability $\mathbb{P}(\theta^\ast\in\hat\Theta)$.
%For this, we employ the extended version of the \emph{leave-out sign-dominated correlation regions} (LSCR) method described in \cite{campi2010Confidence}.
%We summarize the main results of \cite{campi2010Confidence} in the following.
%
%\Oliver{Note which assumptions hold or are imposed}
%
%Select an integer $M$ and construct $M$ unique stochastic binary strings of length $N$, including the zero string, as follows
%\begin{align*}
%	h_{0,1},\ldots,h_{0,N}:=0,\ldots,0\\
%	h_{i,j}\sim p_b,&&j\in\{1,\ldots,N\},
%\end{align*}
%where $p_b$ is the binary probability distribution taking values of 0 or 1 with a probability of 0.5, respectively. Note that unique means $\forall i,j\in\{1,\ldots,N\}: h_{i,0},\ldots,h_{i,N}\neq h_{j,0},\ldots,h_{j,N}$ for $i\neq j$.
%
%We construct the confidence set $\hat\Theta_N$ using the procedure outlined in \cite{campi2010Confidence}, Sec.~III. Based on \cite{campi2010Confidence}, Cor.~2, we can now assign a confidence to $\hat\Theta_N$, given in the following proposition.
%
%For this, we define the following $2M$ functions
%\begin{align}
%	g_{i,j}(\theta)&:=\sum_{k=1}^{N} h_{i,k} u_{k-j} (y_k+\theta_1y_{k-1}-\theta_2u_{k-1}),\label{eq:fun_g}
%\end{align}
%with $i\in\{0,\ldots,M-1\}$ and $j\in\{1,2\}$.
%\begin{proposition}[Confidence set]
%	Assume that $\forall j\in\{1,2\},i\neq 0:\,\mathbb{P}(g_{i,j}(\theta^\ast)=0)=0$.
%	Choose an integer $q\in[1,M/4]$ and sets $\hat{\Theta}_{N,1},\hat{\Theta}_{N,1}\in\Theta$ such that
%%	\begin{itemize}
	%%		\item[a)]
	%		for at least $q$ of $M$ functions $g_{i,j}(\theta)$ as defined in \eqref{eq:fun_g} we have $\forall j\in\{1,2\}:\,g_{i,j}(\theta)>0$.
	%%		\item[b)] for at least $q$ of $M$ functions $g_{i,2}(\theta)$ as defined in \eqref{eq:fun_g} we have $g_{i,2}(\theta)>0$.
	%%	\end{itemize}
%	Then, we find a confidence set
%	\begin{equation}
	%		\hat\Theta=\hat{\Theta}_{N,1}\cap\hat{\Theta}_{N,1}\label{eq:confset}
	%	\end{equation}
%	with a lower bound on the confidence that it contains the true uncertain parameter $\theta^\ast$, namely
%	\begin{equation*}
	%		\mathbb{P}(\theta^\ast\in\hat\Theta) \geq 1-\frac{4q}{M}.
	%	\end{equation*}
%\end{proposition}
%\Oliver{Remark about validity of assumption raised.}



\Oliver{Insert description of how $\hat\theta$ and $\hat\Theta$ are obtained (by gridding. Could use Bobiti \& Lazar (2018)). Include note about introduced conservativeness and assumptions made on e.g. the noise distribution (both minimal or non-existent).}

\Oliver{Establish asymptotic contraction results from paper.}

Through iterative data acquisition and utilizing the provided asymptotic contraction results, successively smaller uncertainty sets can be identified, leading to an overall gain in satisfaction probability growing with $N$.
\color{black}

==> partial_RFF.tex <==
%!TeX root= main.tex

\begin{figure}[htp]
	\centering
	\scalebox{0.9}{	\begin{tikzpicture}
			


			\node[draw,rectangle, fill=gray!50, node distance=6.5cm] (M2) {\begin{minipage}[c]{3.3cm}
					\begin{align*}\SwapAboveDisplaySkip
						\M
					\end{align*}
				\end{minipage}
			};
			
			\node[above of =M2,draw ,rectangle, anchor=south west,fill=lightyellow, node distance=1.6cm] (if2) {\begin{minipage}[c]{2cm}
					Interface
					\begin{align*}\SwapAboveDisplaySkip
						\InF 
					\end{align*}
				\end{minipage}
			};
			\node[above of =M2, draw,rectangle, anchor=south east,fill=lightyellow, node distance=1.6cm] (lif2) {\begin{minipage}[c]{2cm}
					Refinement 
					\begin{align*}\SwapAboveDisplaySkip
					\Refi	\end{align*}
				\end{minipage}
			};
			\path[draw] (if2.south) edge[latex-,right] node{$\x{k} $}(if2.south |- M2.north);
			
			\node[right of =M2, node distance= 3cm](out2){$\y{k}$};
			
			\path[draw] (lif2.south) ++(-0.5cm,0)  edge[latex-,left] node{$ \x{k+1}$} ([xshift=-0.5cm]lif2.south |- M2.north);
			\path[draw] (lif2.south) ++(-0cm,0)  edge[latex-,right] node{$ \x{k}$} ([xshift=-0cm]lif2.south |- M2.north);
			\path[draw] (if2.south) ++(-0.5cm,0)  edge[-latex,left] node{$\ac{k}$} ([xshift=-0.5cm]if2.south |- M2.north);
			
			\node[left of =M2, node distance=2cm,yshift=4cm](MM2) {$\Ca$};
			\node[above of =M2,draw,fill=gray!15, rectangle, minimum width=3.3cm,node distance=5cm, minimum height=1cm] (Ca2) {$\widehat{\Ca}$};
			\path[draw] (Ca2.south) ++(-0.25cm,0)  edge[-latex,right]node{$ \ach{k}$} ([xshift=-0.25cm]Ca2.south |- if2.north);
			\path[draw] (Ca2.south) ++(-1.25cm,0)  edge[latex-,left] node{$ \xh{k+1}$} ([xshift=-1.25cm]Ca2.south |- if2.north);
			\path[draw] (Ca2.south) ++(-.85cm,0)  edge[-latex,right] node{$ \xh{k}$} ([xshift=-.85cm]Ca2.south |- if2.north);
			\path[draw] (Ca2.south) ++(0.5cm,0)  edge[-latex,right] node{$ \ach{k}$} ([xshift=0.5cm]Ca2.south |- if2.north);
			\path[draw] (Ca2.south) ++(1cm,0)  edge[-latex,right] node{$ \xh{k}$} ([xshift=1cm]Ca2.south |- if2.north);
			\begin{scope}[on background layer]
				
				\node[ fill=gray!40, fit= (MM2)(if2)(lif2)(Ca2)](FIt1) {};
				\path[draw] (M2) edge[-latex] (out2);
				
			\end{scope}
		\end{tikzpicture}
	}
	
	
	\caption{Using the conditional lifting for control refinement.  }
	\label{fig:aux_model_3}
\end{figure}

==> relatedWork.tex <==
\subsection{Related work}%\medskip %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% Copied from TAC journal paper on 31. Jan 2024, Oliver Schön
%\noindent\textbf{Related work:}
%{\emph{Abstraction-based approaches:}}
%\textcolor{gray}{\emph{Parametric deterministic systems:}}
\Birgit{Ask Sofie or Sadegh to carefully check this section. I think it is too long and detailed at the moment. Perhaps we can make the reviewers happy with less (complicated) text.}
\noindent\emph{Deterministic systems:}
Data-driven formal approaches
%There are several approaches
for systems with no stochastic state transitions are studied recently in \cite{haesaert2017data,makdesi2021efficient,kazemi2022datadriven}.
%
\new{Notably, \cite{fan2020statistical} presents a verification approach for deterministic systems subject to epistemic uncertainty satisfying signal temporal logic specifications that is based on conformal inference and Gaussian processes (GPs). 
%Conformal methods allow us to quantify prediction intervals of regression models without placing assumptions on the underlying parameter distributions \cite{romano2019conformalized}.
%Extending our approach using conformal inference and GP regression is an interesting direction for further research. Furthermore, state-dependent confidence parameters can be obtained using quantile regression \cite{romano2019conformalized} or locally-weighted conformal inference \cite{lei2018distribution}.
One major issue with conformal methods is that available results can generally only provide rigorous guarantees for infinitely many samples \cite{romano2019conformalized}. In contrast, we obtain finite-sample guarantees using Bayesian linear regression.
% \Birgit{Shorten this new part. In my opinion the part Conforming methods ....  conformal inference [], can be removed.}
}

\noindent\emph{Abstraction-based approaches:}
%\textcolor{gray}{\emph{Uncertain stochastic systems:}}
%\textcolor{gray}{\emph{Two-player games finite state:}}
For stochastic systems, one approach for dealing with epistemic uncertainty is to model it as a stochastic two-player game, where the objective of the first player is to create the best performance considering the worst-case epistemic uncertainty.
%\pdfmargincomment{How is that different to what we are doing?}
The literature on solving stochastic two-player games is relatively mature for finite state systems \cite{chatterjee2016perfect,chatterjee2012survey}.
%
%\textcolor{gray}{\emph{Two-player games continuous state:}}
There is a limited \new{body} of papers addressing this problem for continuous-state systems. The papers \cite{majumdar2021symbolic,majumdar2020symbolic} look at satisfying temporal logic specifications on nonlinear systems utilizing mu-calculus and space discretization. The results rely on direct access to the full state and are hence incompatible with model order reduction techniques.
%
%\new{Conversely, the authors in \cite{kazemi2022datadriven} compute a growth bound of the unknown system and design controllers founded on estimating a bound on the Lipschitz constant of the system.}
%
%\textcolor{gray}{\emph{Interval MDPs:}}
The work \cite{Badings2022epistemicUncert} addresses epistemic uncertainty in stochastic systems by abstracting the system to an interval Markov decision process (MDP) and is limited to finite horizons, reach-avoid specifications, and linear systems.
%\textcolor{gray}{\emph{Scenario optimization:}}
%\Oliver{Many approaches limited to bounded stochastic noise!}
Similarly, \cite{Lavaei2022DDMDP} extends upon this by constructing an interval MDP for uncertain nonlinear systems by solving a scenario optimization problem. This is helpful when only data of the system is available or the dynamics are very complex.
\new{The authors of the papers \cite{Jackson2020safety, jiang2022safe} use GPs instead of scenario optimization. This is extended with deep kernel learning in \cite{reed2023promises}, where the GP kernel is augmented with a neural network preprocessing its inherent feature map.
}
\new{Controllers for systems captured as stochastic neural network dynamic models (NNDMs) are designed in \cite{adams2022nndm} by translating the NNDMs to interval MDPs.
The starting point, however, is the NNDM and no guarantees on the correctness of the learned model w.r.t. to the data-generating system are considered, rendering the approach only robust from a model-based perspective.
}
Capturing epistemic uncertainty using interval MDPs relies on the assumption that the epistemic uncertainty is state-wise independent, leading to inconsistent and overly conservative results.
In contrast, we relate epistemic uncertainty explicitly using parametric MDPs.
\new{Furthermore, approaches based on interval MDPs are generally limited to finite horizons on requirements such as safety if the noise is unbounded.} 
%\Birgit{This is a crucial point to make! Most approaches do not work for stochastic systems where the noise is additive and unbounded, \emph{especially} when the specifications have a finite horizon. Perhaps we can try to categorize the different techniques and shorten by saying: we have deterministic approaches [],[],[]. Approaches that work based on ...., but they are limited to ....}
%
%\textcolor{gray}{\emph{Model-free:}}
%\textcolor{gray}{\emph{Reinforcement learning:}}
\new{In an effort of reducing the number of required assumptions, \cite{thorpe2022cmechance} use conditional mean embeddings (CMEs) to embed the conditional distribution of a non-Markovian random trajectory into an reproducing kernel Hilbert space (RKHS). 
%	Whilst this direction seems generally promising, 
%	the authors do not provide any rigorous end-to-end guarantees for their results and obtain their approximate chance constrained optimization problem by using an empirical CME and disregarding its statistical correctness. 
However, the authors obtain their approximate chance-constrained optimization problem by using an empirical CME without providing guarantees of its statistical correctness.
%	\Birgit{Too harsh? Reformulate}
The authors of \cite{romao2023distributionally} provide a similar distributionally-robust scheme, leaving the necessary theoretical results for quantifying the size of the required ambiguity set for future work.
}



\noindent\emph{Abstraction-free approaches:} %{\emph{Abstraction-free approaches:}}
Latest work in the area of abstraction-free approaches develop control barrier certificates (CBCs) that are based on constructing a set of feasible models \cite{Cohen2022RCBF}.
Similarly, adaptive control for continuous-time control-affine parametric systems using so-called unmatched control barrier functions is studied in \cite{Lopez2022UnmatchCBC}.
\new{In \cite{salamati2024data}, the authors find CBCs using robust scenario optimization. Whilst this necessitates them to sample transitions between every pair of partitions multiple times, incurring a high sample burden, they also require knowledge of the Lipschitz constants of several intermediate functions.}
%Analogous to our approach, the authors generate a family of control barrier functions and use online parameter adaptation to select a safety controller from the obtained set.
Whilst CBCs are potentially more scalable than abstraction-based solutions, finding a valid CBC for systems with non-control-affine and non-polynomial dynamics is generally hard. Even more, CBCs for specifications beyond simple reachability yields, e.g., sequential reachability problems \cite{anand2021CBComegaregular}, greatly impeding their applicability.
%\Oliver{Add \cite{Ameneh2023DataDriven}?}
Further work on model-free reinforcement learning studies synthesizing robust controllers for temporal logic specifications without constructing a model of the system \cite{kazemi2020fullLTL,lavaei2020RL}.
%Moreover, the work \cite{Cohen2022RCBF} is limited to polyhedral over-approximations of the credible set that introduces another degree of conservatism.
%Similarly, adaptive control for continuous-time control-affine parametric systems using the so-called unmatched control barrier functions is studied in \cite{Lopez2022UnmatchCBC}. Analogous to our approach, the authors generate a family of control barrier functions and use online parameter adaptation to select a safety controller from the obtained set. However, the work is limited to forward invariance specifications.
%\color{black}
\new{An approach based on computing reachable sets leverages random set theory to obtain infinite-sample guarantees \cite{lew2021sampling}. 
%	Analyzing convergence rates is left for future work. \Birgit{Same for us, right? If yes, remove this sentence. }
Similarly, further work construct reachable sets efficiently using knowledge of a growth bound \cite{ajeleye2023data}, and GPs under the assumption of known bounds on the unknown dynamics components \cite{cao2022efficient}, respectively.
There exist a body of work on verifying models based on neural networks \cite{harapanahalli2023forward, jafarpour2023interval}. However, similar as mentioned before, no guarantees of the correctness of the data-driven model w.r.t. the data-generating system are provided.
}

\noindent\emph{Other related work:} %\Birgit{alt: Other related work:}
\new{There is a large body on model predictive control (MPC) based approaches trying to address the challenges arising from uncertain systems \cite{dyro2021particleMPC, sinha2022adaptive}. For example, in \cite{dyro2021particleMPC}, the authors propose a particle MPC solves using sequential convex programming. Note that these approaches can generally not give any guarantees for the robustness of the resulting controller.
As one example of a wealth of work on planning, probabilistically safe planning under uncertain human interactions via a real-time Bayesian framework is studied in \cite{fisac2018probabilistically}.}
\new{There is a growing body of work on utilizing polynomial chaos expansion to propagate stochastic distributions through dynamics, which is to date mainly limited to linear systems \cite{pan2023polychaos, kim2013polychaos, seshadribayesian}.}

Our approach utilizes the techniques from the system identification literature to compute parameter sets with respect to a given confidence for stochastic systems. We then build theoretical foundation on the concepts presented in \cite{haesaert2017verification,haesaert2020robust} to design robust controllers using abstraction methods that are compatible with both model order reduction and \new{space} discretization.

%One approach of dealing with epistemic uncertainty is to model it as an adversarial player in the problem formulation. The synthesis problem can be cast as a max-min optimization where the goal of the controller (max player) is to maximize the satisfaction probability for all possible trajectories of the system under epistemic uncertainty. This then becomes a stochastic two-player game where the objective of the first player is to create the best performance considering the worst-case uncertainty. The literature on solving stochastic two-player games is relatively mature for finite state systems \cite{chatterjee2012survey,chatterjee2016perfect}. However, there is a limited number of papers addressing this problem for continuous-state systems. The paper \cite{svorevnova2017temporal} looks at satisfying temporal logic specifications on linear systems using abstraction as a finite two-player stochastic game. The papers \cite{majumdar2020symbolic,majumdar2021symbolic} generalize the approach to nonlinear systems utilizing mu-calculus for computing the approximately optimal controller.


%Another approach of dealing with this problem {\color{red} .... }.

% references on continuous time models
%\red{[consider removing the next two sentences]}\Oliver{Removed bc not relevant and didn't fit the flow}\new{\emph{Continuous-time stochastic systems:}} For  \emph{continuous-time} stochastic systems with uncertainty results are available for robust stabilization \cite{li2017robust,zhang2005quadratic}. %. This includes \new{Papers covering the robust stabilization of uncertain stochastic systems include \cite{li2017robust,zhang2005quadratic}.}
%The paper \cite{li2017robust} studies the problem of robust stabilization of uncertain stochastic systems when the controller is in the form of discrete-time state feedback. The model of the system includes uncertainty in both its drift and diffusion functions. Robust quadratic stabilization of stochastic uncertain systems is discussed in \cite{zhang2005quadratic} while considering both state and output feedback controllers and assuming matrix uncertainty with bounded norm. Linear matrix inequalities are formulated as conditions for robust quadratic stabilization of the system.
%Uncertain stochastic systems with time-varying delay are studied in \cite{niu2005robust}.
%, where the system includes both time-varying parameter uncertainties and unknown but bounded nonlinear functions.
%The authors propose a sliding mode controller and use linear matrix inequalities to guarantee the global stochastic stability of the closed-loop system.

%\Oliver{Suggesting cutting more of the related work to stay within page limit.}


%\red{The step from the previous paragraph to this sentence seems difficult. It could make more sense to switch the order of this subsection. First talk about the literature for deterministic systems and then talk about stochastic systems, point out what is missing and tell them we will do that.}
%\new{In this paper, however, the scope lies on general discrete-time nonlinear stochastic systems.}
%\Oliver{First param uncert determ sys. Then what exists so far for stoch sys. Then show gap and that this paper fills that gap.}
%Correct-by-design controllers have been developed in \cite{haesaert2017data} for deterministic linear time-independent systems. Extensions to more complex specification sets have been provided in \cite{salamati2020data}. Synthesizing symbolic models directly from data for monotone systems is discussed in \cite{makdesi_data}.
%https://www.theses.fr/s255864

%
%
%\Sadegh{use in the full version}
%The research on system identification is relatively mature with a diverse set of algorithms and tools in identifying a model for the system using collected data \cite{ljung1998system}. From a parametrized class of models, the best parameter values are computed using a finite set of data from the system. Confidence sets for the parameters can be quantified with finite data sets based on the results in \cite{campi2005guaranteed,prando2016classical,khorasani2018non}.
%42. Prando, G., Romeres, D., Pillonetto, G., Chiuso, A.: Classical vs. Bayesian methods for linear system identification: Point
%estimators and credible sets. In: 2016 European Control Conference (ECC). pp. 1365?1370 (2016).
%43. Campi, M.C., Weyer, E.: Guaranteed non-asymptotic credible regions in system identification. Automatica. 41,
%1751?1764 (2005).
%44. Khorasani, M.M., Weyer, E.: Non-Asymptotic Confidence Regions for Errors-In-Variables Systems. IFAC-PapersOnLine.
%51, 1020?1025 (2018).
%45. Kieffer, M., Walter, E.: Guaranteed characterization of exact non-asymptotic credible regions in nonlinear
%parameter estimation. IFAC Proceedings Volumes. 46, 56?61 (2013).
%The credible set quantifies the remaining uncertainty about the model. We refer to this uncertainty as the epistemic uncertainty.
%\color{blue!70!black}

%The literature on addressing correct-by-design control for systems subject to aleatoric uncertainty, i.e., stochastic systems, is comparatively mature [...], as is the literature on epistemic uncertainty for deterministic systems [...].

%Paper also addressing epistemic uncertainty for stochastic systems: \cite{Badings2022epistemicUncert} using interval MDPs. Robust satisfaction probability only for finite horizons, reach-avoid specifications, and linear systems, but handles potentially unknown noise distributions.
%\hrule
% uCBC (CBCs are hard to generate over hybrid spaces, which would be needed to address the same type of specifications).

%In summary, our approach distinguishes itself from hitherto presented in the literature in the following features: \pdfmargincomment{Do we want a list like this and if yes, in what format?}
%\begin{itemize}
%	\item Robust control synthesis for complex scLTL specifications over possibly infinite horizons and hybrid state spaces \cite{haesaert2020robust};
%	\item compatibility with standard model order reduction techniques utilizing the results from \cite{VanHuijgevoort2020SimQuant}, Sec.~5;
%%	yielding a lower dimensional continuous-state model. This aids in alleviating the computational burden of the subsequent controller synthesis.
%%	\item compatibility with compositional approaches \cite{lavaei2021automated};
%	\item applicability to nonlinear systems using the results from \cite{huijgevoort2022piecewiseaffineabstraction}; and
%	\item accessible in use and adaptation, being based on the publicly available tool \textsl{SySCoRe}\footnote{Available at $<$URL$>$.} \cite{}.
%\end{itemize}
%\color{black}
